Harness Annealing: Learning to Act with Less External Control

Language agents rely on external harnesses to track state, organize workflows, and verify answers. Beyond providing tools and information, these harnesses supply control decisions about what to investigate, whether to revise, and when to stop. Training on successful harness-supported trajectories can improve task performance while leaving these decisions dependent on runtime intervention. We ask whether harness-supported experience can also teach the model to make these decisions, allowing the division of control to change as the model learns. We call this objective harness internalization: learning to assume specified control responsibilities while retaining task performance after the corresponding support is withdrawn. We introduce HARNESS ANNEALING TRAINING (HAT), which combines explicit control supervision with a curriculum over teacher trajectories collected under progressively weaker harnesses. Experiments with 9B and 35B models on SWE-QA and SWE-QA-Pro evaluate every checkpoint under four deployment harnesses. Selected annealed checkpoints operating with tools alone achieve scores close to those of their respective starting checkpoints deployed with the full harness. The benefits vary with model scale and deployment configuration, and further annealing does not uniformly improve performance. These findings suggest that harness-supported experience can help reduce the runtime control required by a trained agent.

==> figures/annealing_protocol_figure.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/annealing_protocol.pdf}
  \caption{\textbf{Harness Annealing alternates control-layer removal, consolidation, and measurement.}
  Repository access and the tool interface remain fixed throughout; answer checking, workflow selection, and a coupled state-control layer are removed in sequence.  Training begins with Verify-guided decision records.  Each subsequent stage targets decisions from the weaker configuration while replaying earlier decisions and initializes from the preceding adapter.  Every checkpoint is then evaluated under every fixed deployment harness; the pre-specified transition cells measure transfer, while the remaining cells measure retention and specialization.}
  \label{fig:protocol}
\end{figure*}


==> sections/04_results_new.tex <==
\section{Results}
\label{sec:results}

\subsection{Controlled removal exposes harness dependence}

\textbf{A fixed checkpoint exhibits a measurable dependency profile across runtime controls.}
For the Verify-trained checkpoint, SWE-QA ranges from 71.99 with Tools alone to 77.47 under Workflow, although the weights, repository, tools, and evaluator are identical.  The nominally strongest configuration is not always best: adding answer verification changes the score to 75.70.  Removing runtime control therefore does not merely subtract a fixed bonus; it changes the sequential policy that the model--harness system executes.  Reporting only the score obtained behind the training harness conceals both the magnitude and the shape of this dependence.

The legacy Base evaluation was collected under a different protocol and is not pooled into the main matrix.  The present attribution claim is therefore restricted to how trained checkpoints respond to controlled support removal; it is not a complete decomposition of the unadapted model--harness system.

\subsection{Decision-segmented supervision yields stronger cross-harness transfer}

\textbf{Materializing decision boundaries is associated with stronger transfer than serialized rollout supervision.}
The legacy V4 cohort pairs two constructions of the same successful rollouts.  Direct supervision serializes a rollout as one multi-turn training example; Layered supervision materializes its decision boundaries as separately sampled records.  Both autoregressive objectives condition each assistant target on the preceding trajectory prefix.  Layered additionally changes prefix repetition, sampling frequency, and the effective loss weight assigned to each decision.  The source harness, question IDs, and underlying experience are held fixed, but total target tokens and optimizer exposures are not yet matched.

\input{tables/direct_layered}

Table~\ref{tab:direct-layered} reports the complete cross-harness matrices rather than only their averages.  The missing cells matter.  Under Tools deployment, the four Direct models score only 16.51--32.45 on SWE-QA and 16.69--34.74 on SWE-QA-Pro; the corresponding Layered models score 53.73--72.48 and 59.75--77.52.  Direct supervision can therefore look adequate behind a supportive harness while failing precisely where the policy must reconstruct control from its own history.

Across all four training sources, Layered supervision improves the four-deployment average by 12.16--25.23 points on SWE-QA and 13.32--22.68 points on SWE-QA-Pro.  The largest margin occurs for Verify-source data.  One plausible explanation is that separately materializing the stop-versus-search boundary gives rare consequential decisions more optimization weight.  The current comparison, however, evaluates the complete decision-segmented construction.  A target-token- and update-matched control is required before attributing the gain specifically to boundary supervision rather than additional prefix exposure or reweighting.

Because the V4 and V5 cohorts differ in generation limits, retry accounting, and judge provenance, we use this result to select the training representation and do not pool the two cohorts numerically.

\subsection{Annealing shifts control toward weaker support}

\textbf{Task performance remains in a similar band across three successive reductions in runtime control.}
Table~\ref{tab:main-results} contains the full checkpoint-by-deployment cross-product.  Each row is the removal profile of one checkpoint, and each successive row follows an induction stage under weaker support.  The red cells are specified by the experimental sequence rather than selected post hoc: each evaluates the newly trained checkpoint after the target runtime component has been removed.

\input{tables/main_results}

The Verify-trained checkpoint reaches 77.47 on SWE-QA and 76.87 on SWE-QA-Pro under Workflow.  After Workflow-targeted training, the State deployment reaches 77.15 and 77.96, respectively.  After State-targeted training, Tools alone reaches 77.00 and 77.73.  These endpoint scores establish retention of task performance after the corresponding runtime layer is absent.  Whether the policy also reconstructs the removed control behavior---rather than reaching similar answers through a different policy---is tested by the pre-specified trajectory analysis in Appendix~\ref{app:trajectory-analysis}.

Figure~\ref{fig:heatmaps} shows the pre-specified transition cells as a staircase toward weaker deployment support.  Relative to the Verify-trained checkpoint, the State-targeted checkpoint improves Tools-only performance by 5.01 points on SWE-QA and 3.09 points on SWE-QA-Pro, while Verify performance changes by only $+0.75$ and $+0.05$.  The weak-support gain is therefore not obtained by sacrificing performance whenever stronger support remains available.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.49\textwidth]{figures/heatmap_sweqa.pdf}\hfill
%   \includegraphics[width=0.49\textwidth]{figures/heatmap_sweqapro.pdf}
%   \caption{\textbf{Scores at the three pre-specified scaffold-removal transitions.}
%   Red outlines mark evaluation after removing answer verification, workflow control, and the coupled state-control layer.  The final Tools-targeted stage is shown as a continuation of the training recipe rather than a fourth layer removal.}
%   \label{fig:heatmaps}
% \end{figure*}

The transfer is cumulative, not cell-wise monotonic.  From the Workflow-targeted checkpoint to the State-targeted checkpoint, Tools changes by $-0.41$ on SWE-QA and $+0.67$ on SWE-QA-Pro, even though the latter checkpoint is more robust overall.  The evidence supports transfer under the complete staged recipe; an equal-token joint mixture is still required to separate curriculum order from additional data and optimization.

\subsection{Performance peaks at an intermediate evaluated stage}

\textbf{Training under the least controlled configuration does not improve aggregate performance in the observed run.}
If continued optimization under weaker support necessarily improved cross-harness robustness, the Tools-targeted stage should not lower the aggregate.  The observed final stage does not support that monotonic prediction.

\input{tables/aggregate_results}

The State-targeted checkpoint has the best mean on SWE-QA (76.63), SWE-QA-Pro (77.71), and their equal-weight aggregate (77.17), together with the strongest worst-configuration score (76.43).  The subsequent Tools-targeted stage lowers every SWE-QA cell by 0.70--2.29 points and reduces the benchmark mean by 1.63.  SWE-QA-Pro is more stable, but its mean still falls by 0.23.  Across both benchmarks, the loss is 0.93 points.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/annealing_curve.pdf}
  \caption{\textbf{Cross-harness robustness across the evaluated training stages.}
  Each point aggregates one checkpoint over the four fixed deployment harnesses.  Under the current data mixture and single-seed recipe, the State-targeted checkpoint has the highest mean and worst-configuration score; the Tools-targeted continuation lowers these descriptive quantities.}
  \label{fig:curve}
\end{figure}

The State-targeted checkpoint is therefore the best empirical point among the stages evaluated under this recipe, not evidence for a universal optimum.  Lower-quality Tools targets, insufficient replay, adapter interference, or specialization may explain the final regression.  The score matrix identifies where the observed decline begins but does not distinguish these mechanisms; trajectory analysis and replay/data-quality ablations are needed for that attribution.

\subsection{The final stage shortens search on SWE-QA}

\textbf{The observed decline is associated with less interaction, not more looping.}
On the 720 SWE-QA questions, the Tools-targeted stage reduces mean tool calls by 1.75, 1.77, 2.86, and 2.30 under Tools, State, Workflow, and Verify, respectively; episode length falls by 0.69--1.11 steps.  Completion remains nearly saturated and loops do not increase.  Lexical F1 rises by 0.28 points under Tools but falls by 0.63 under State, 0.71 under Workflow, and 1.37 under Verify.  These are descriptive changes on the fixed evaluation set.  This pattern is consistent with less exhaustive search and weakest-interface specialization, but evidence-coverage labels, final-attempt matching, and per-example judge outputs are still needed for a causal account.

\textbf{The same shift is present in the supervision.}
Across the complete post-cleaning mixtures, mean tool calls fall from 15.97 to 15.22 to 13.40 and mean search calls from 5.50 to 4.68 to 4.17 as training proceeds through Workflow-, State-, and Tools-targeted stages.  Mean observed tool-result content falls from 91.5K to 88.6K to 78.3K characters, while explicit reasoning grows from 369 to 409 to 428 words.  The contrast is larger within the new target data than in replay: Tools targets contain 11.78 calls, 3.51 searches, and 70.1K observed characters, compared with 14.95, 4.42, and 87.7K for State targets.  Their available upstream judge mean is also lower (88.8 versus 90.8).  The final stage therefore changes the demonstrated allocation of effort rather than merely deleting a state field: it places more weight on internal synthesis and less on acquiring external evidence.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/behavior_mechanism.pdf}
  \caption{\textbf{The final training distribution induces a shorter, heterogeneous search policy.}
  \textbf{Left:} measured properties of the complete cleaned training mixtures.  Observation is tool-result text, not model context length.  \textbf{Right:} complete-cohort SWE-QA outcomes for the State-targeted to Tools-targeted transition.  Compression means at least two fewer tool calls; the useful/harmful split uses a $\pm2$-point lexical-F1 margin and is diagnostic until per-example judge outputs are recovered.}
  \label{fig:behavior-mechanism}
\end{figure*}

\textbf{Shorter execution is sometimes internalization and sometimes premature commitment.}
Figure~\ref{fig:behavior-mechanism} conditions compression on answer quality.  On SWE-QA, the fraction of episodes with harmful compression increases with deployment support, from 16.1\% under Tools to 17.6\% under State, 18.6\% under Workflow, and 20.3\% under Verify.  Useful compression moves in the opposite direction, from 19.4\% under Tools to 16.7\% under Verify.  Thus the later checkpoint appears specialized toward the least structured interface and underuses workflow and verification support when it remains available.  This monotone pattern does not appear on SWE-QA-Pro, so we treat it as a benchmark-dependent mechanism rather than a universal property of annealing.

Conservatively matched raw trajectories make the distinction concrete.  On \texttt{scikit-learn-00005}, the Tools-targeted checkpoint removes repeated unavailable commands, recovers from the tool mismatch, reaches the implementation and tests, and improves its answer.  On \texttt{conan-00011}, it stops after locating but before reading the relevant file, then substitutes plausible but nonexistent symbols for the implementation it did not observe.  The relevant outcome is therefore \emph{evidence-adjusted efficiency}: work saved while retaining the evidence required for a correct answer.  Appendix~\ref{app:trajectory-analysis} reports final-attempt coverage and the complete paired feature table; the cases follow a frozen behavior-and-score sampling rule rather than post-hoc visual selection.

\FloatBarrier


==> tables/aggregate_results.tex <==
\begin{table}[t]
\caption{\textbf{Cross-harness aggregate performance.} The shaded row is the best observed stage under the current recipe. Combined weights the two benchmarks equally; $\Delta$ is relative to the Verify-trained checkpoint.}
\label{tab:aggregate}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Checkpoint & SWE-QA & Pro & Combined & $\Delta$ & Worst \\
\midrule
Verify-trained          & 75.28 & 76.89 & 76.08 & --    & 71.99 \\
Workflow-targeted & 76.33 & 77.13 & 76.73 & +0.65 & 75.10 \\
\stopcell{State-targeted} & \stopcell{\textbf{76.63}} & \stopcell{\textbf{77.71}} & \stopcell{\textbf{77.17}} & \stopcell{\textbf{+1.09}} & \stopcell{\textbf{76.43}} \\
Tools-targeted    & 75.00 & 77.48 & 76.24 & +0.16 & 74.16 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/decision_probe_transitions.tex <==
\begin{table}[H]
\caption{\textbf{Only the State-to-Tools transition improves both stopping diagnostics immediately.}
Changes in percentage points, later minus earlier checkpoint, with the
weaker input fixed. Positive values mean improvement. These are differences
of the scores computed on the same reference-state set, not new rollouts.}
\label{tab:probe-transitions}
\centering
\small
\renewcommand{\arraystretch}{1.18}
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrr@{}}
\toprule
Training transition & Fixed input & \shortstack{Stop/continue\\F1} & \shortstack{Late/final\\accuracy} & \shortstack{Next-tool\\accuracy} \\
\midrule
Verify to Workflow & Workflow & $-1.09$ & $-1.88$ & $-0.31$ \\
Workflow to State & State & $-0.69$ & $-1.25$ & $+0.31$ \\
State to Tools & Tools-only & $+3.85$ & $+4.38$ & $+0.63$ \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/direct_layered.tex <==
\begin{table*}[t]
\caption{\textbf{Direct and Layered supervision produce different cross-harness transfer profiles.}
Each block contains the unchanged Base policy followed by models trained from Tools, State, Workflow, or Verify data.  Columns are fixed inference harnesses, and bold marks the matched training--deployment condition.  The Base row is repeated to make each five-row block self-contained; ``--'' denotes an unavailable legacy SWE-QA-Pro Base score.}
\label{tab:direct-layered}
\centering
\scriptsize
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llrrrrrrrr@{}}
\toprule
& & \multicolumn{4}{c}{SWE-QA inference harness} & \multicolumn{4}{c}{SWE-QA-Pro inference harness} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
Supervision & Training source & Tools & State & Workflow & Verify & Tools & State & Workflow & Verify \\
\midrule
\multirow{5}{*}{Direct}
 & Base     & 59.93 & 62.92 & 67.28 & 66.79 & --    & --    & --    & --    \\
 & Tools    & \textbf{32.45} & 65.83 & 62.29 & 59.65 & \textbf{34.74} & 65.69 & 66.28 & 64.02 \\
 & State    & 16.76 & \textbf{57.83} & 58.98 & 61.30 & 17.88 & \textbf{66.95} & 62.58 & 62.63 \\
 & Workflow & 17.91 & 64.15 & \textbf{64.60} & 61.71 & 18.43 & 66.89 & \textbf{66.95} & 66.88 \\
 & Verify   & 16.51 & 60.21 & 61.28 & \textbf{62.19} & 16.69 & 68.88 & 67.23 & \textbf{64.02} \\
\midrule
\multirow{5}{*}{Layered}
 & Base     & 59.93 & 62.92 & 67.28 & 66.79 & --    & --    & --    & --    \\
 & Tools    & \textbf{72.48} & 75.18 & 75.78 & 72.91 & \textbf{77.52} & 78.28 & 78.02 & 76.72 \\
 & State    & 53.73 & \textbf{69.23} & 68.56 & 66.18 & 59.75 & \textbf{71.53} & 68.43 & 66.21 \\
 & Workflow & 62.27 & 67.52 & \textbf{72.08} & 55.14 & 68.70 & 73.21 & \textbf{68.97} & 61.54 \\
 & Verify   & 71.99 & 75.94 & 77.47 & \textbf{75.70} & 74.64 & 77.81 & 76.87 & \textbf{78.25} \\
\bottomrule
\end{tabular}%
}
\end{table*}


==> tables/harnessx_dimensions.tex <==
\refstepcounter{table}
\label{tab:harnessx-dimensions}
\noindent\textbf{Table \thetable: HarnessX behavioral dimensions used in this study.} The taxonomy is a composition substrate, not the source of our harness-level names.
\begin{center}
\footnotesize
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{@{}clp{0.29\textwidth}p{0.30\textwidth}@{}}
\toprule
Dim. & HarnessX behavior dimension & General control surface & Role in our SWE-QA study \\
\midrule
D1 & Model selection & Provider routing and role assignment & Fixed Qwen3.5-9B family; checkpoints vary only through training. \\
D2 & Context assembly & System prompt, history construction, user wrapping & Level-specific prompts; progressive state and workflow cues. \\
D3 & Memory & Extract, retain, retrieve across steps/sessions & Sliding-window retrieval enters at H2 \textsc{State}. \\
D4 & Tools & Tool registry, schema, filtering & Read/Grep/Glob/read-only Bash enter at H1 \textsc{Tools}. \\
D5 & Sandbox & Where tool side effects materialize & Fixed pinned checkout; not an annealed capability. \\
D6 & Evaluation/reward & Judges, verifiers, process/outcome rewards & Non-oracle answer verifier enters at H4 \textsc{Verify}; gold judge remains external. \\
D7 & Control/safety & Loop, budget, guard, correction policies & Fixed read-only/token guard plumbing; loop detection enters at H2 \textsc{State}. \\
D8 & Observability & Event traces, metrics, checkpoints, recovery & Fixed journal/tracer; supplies trajectories and failure diagnostics. \\
D9 & Training bridge & Trajectory conversion for SFT/RL & We export layered step-level SFT records and replay mixtures. \\
\bottomrule
\end{tabular}
\end{center}


==> tables/implementation_mapping.tex <==
\refstepcounter{table}
\label{tab:implementation-map}
\noindent\textbf{Table \thetable: Implementation mapping retained for reproducibility.} Internal level/checkpoint abbreviations are not used as conceptual names in the main paper.
\begin{center}
\small
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lll}
\toprule
Paper harness & Legacy code/config level & Training checkpoint mapping \\
\midrule
H0 Direct & legacy h0 / QH0 & -- \\
H1 Tools & legacy h2 / QH2 & Tools-targeted; legacy H6542 \\
H2 State & legacy h4 / QH4 & State-targeted; legacy H654 \\
H3 Workflow & legacy h5 / QH5 & Workflow-targeted; legacy H65 \\
H4 Verify & legacy h6 / QH6 & Verify-trained; legacy H6 adapter \\
\bottomrule
\end{tabular}
\end{center}


==> tables/main_results.tex <==
\begin{table*}[t]
\caption{\textbf{Every training checkpoint is evaluated under every deployment configuration.} Red cells mark the three pre-specified scaffold-removal transitions; bold values are column maxima.  Each targeted checkpoint continues training from the row above.}
\label{tab:main-results}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrrrrrr@{}}
\toprule
Benchmark & Training checkpoint & Tools & State & Workflow & Verify & Mean & Worst \\
\midrule
\multirow{4}{*}{SWE-QA}
 & Verify-trained          & 71.99 & 75.94 & \frontiercell{77.47} & 75.70 & 75.28 & 71.99 \\
 & Workflow-targeted & \textbf{77.41} & \frontiercell{77.15} & 75.10 & 75.66 & 76.33 & 75.10 \\
 & State-targeted    & \frontiercell{77.00} & 76.62 & 76.43 & \textbf{76.45} & \textbf{76.63} & \textbf{76.43} \\
 & Tools-targeted    & 76.30 & 75.12 & 74.43 & 74.16 & 75.00 & 74.16 \\
\addlinespace[2pt]
\midrule
\multirow{4}{*}{SWE-QA-Pro}
 & Verify-trained          & 74.64 & 77.81 & \frontiercell{76.87} & 78.25 & 76.89 & 74.64 \\
 & Workflow-targeted & 77.06 & \frontiercell{77.96} & 75.97 & 77.54 & 77.13 & 75.97 \\
 & State-targeted    & \frontiercell{77.73} & 77.83 & 76.98 & \textbf{78.30} & \textbf{77.71} & 76.98 \\
 & Tools-targeted    & 77.12 & 77.40 & \textbf{77.94} & 77.47 & 77.48 & \textbf{77.12} \\
\bottomrule
\end{tabular*}
\end{table*}


==> tables/paired_behavior.tex <==
\begin{table}[H]
\setlength{\abovecaptionskip}{0pt}
\caption{\textbf{Shorter SWE-QA runs do not yield higher lexical F1; Pro changes are smaller and mixed.}
Tools-targeted minus State-targeted, paired by question and deployment
harness. $N$ is the number of matched episode pairs. Counts are mean
differences; F1 differences are percentage points, not LLM-judge scores.}
\label{tab:paired-behavior}
\centering
\small
\renewcommand{\arraystretch}{1.18}
\begin{center}
\vspace{+0.2cm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrrrr@{}}
\toprule
Benchmark & Harness & $N$ & $\Delta$ Steps & $\Delta$ Calls & $\Delta$ Read & $\Delta$ Lexical F1 \\
\midrule
SWE-QA & Tools & 405 & $-0.93$ & $-2.38$ & $-0.43$ & $-0.01$ \\
 & State & 398 & $-0.70$ & $-1.44$ & $+0.06$ & $-0.80$ \\
 & Workflow & 343 & $-0.67$ & $-2.50$ & $-0.57$ & $-0.74$ \\
 & Verify & 357 & $-0.62$ & $-2.13$ & $-1.01$ & $-1.20$ \\
\addlinespace[4pt]
SWE-QA-Pro & Tools & 149 & $+0.67$ & $+0.11$ & $-0.21$ & $+0.39$ \\
 & State & 122 & $+0.01$ & $-0.14$ & $+0.06$ & $+0.24$ \\
 & Workflow & 100 & $-0.13$ & $-0.64$ & $+0.27$ & $+0.37$ \\
 & Verify & 117 & $-0.09$ & $-1.48$ & $-0.32$ & $+0.91$ \\
\bottomrule
\end{tabular*}
\end{center}
\end{table}


==> tables/training_behavior.tex <==
\begin{table}[H]
\caption{\textbf{Behavioral statistics of the cleaned 9B training mixtures.}
Values are means per multi-turn training record, except the record counts.
Calls are parsed from cleaned function-call targets; searches are the
\texttt{Grep}/\texttt{Glob} subset. Reasoning counts whitespace-delimited words
inside \texttt{<think>} blocks, and observations count serialized tool-result characters.}
\label{tab:training-behavior}
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Stage mixture & Records & Tool calls & Searches & \shortstack{Reasoning\\words} & \shortstack{Observation\\chars} \\
\midrule
Workflow-targeted & 1,775 & 15.97 & 5.50 & 369 & 91,499 \\
State-targeted & 2,049 & 15.22 & 4.68 & 409 & 88,630 \\
Tools-targeted & 2,291 & 13.40 & 4.17 & 428 & 78,345 \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/trajectory_coverage.tex <==
\begin{table}[H]
\caption{\textbf{Matched-trajectory coverage for the final-stage comparison.}
Cells report matched raw episodes / evaluated questions for each checkpoint
and deployment harness. These are analysis-coverage counts, not completion
or success counts. Matching follows the rule described above.}
\label{tab:trajectory-coverage}
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrrr@{}}
\toprule
Checkpoint & Benchmark & Tools & State & Workflow & Verify \\
\midrule
State-targeted & SWE-QA & 476/720 & 486/720 & 434/720 & 442/720 \\
State-targeted & SWE-QA-Pro & 171/260 & 157/260 & 142/260 & 143/260 \\
\addlinespace[3pt]
Tools-targeted & SWE-QA & 523/720 & 496/720 & 454/720 & 469/720 \\
Tools-targeted & SWE-QA-Pro & 186/260 & 150/260 & 136/260 & 160/260 \\
\bottomrule
\end{tabular*}
\end{table}

